Hierarchical surrogate-based Approximate Bayesian Computation for an electric motor test bench

Inferring parameter distributions of complex industrial systems from noisy time series data requires methods to deal with the uncertainty of the underlying data and the used simulation model. Bayesian inference is well suited for these uncertain inverse problems. Standard methods used to identify uncertain parameters are Markov Chain Monte Carlo (MCMC) methods with explicit evaluation of a likelihood function. However, if the likelihood is very complex, such that its evaluation is computationally expensive, or even unknown in its explicit form, Approximate Bayesian Computation (ABC) methods provide a promising alternative. In this work both methods are first applied to artificially generated data and second on a real world problem, by using data of an electric motor test bench. We show that both methods are able to infer the distribution of varying parameters with a Bayesian hierarchical approach. But the proposed ABC method is computationally much more efficient in order to achieve results with similar accuracy. We suggest to use summary statistics in order to reduce the dimension of the data which significantly increases the efficiency of the algorithm. Further the simulation model is replaced by a Polynomial Chaos Expansion (PCE) surrogate to speed up model evaluations. We proof consistency for the proposed surrogate-based ABC method with summary statistics under mild conditions on the (approximated) forward model.

==> Plots/colorbar_color.tex <==

\begin{tikzpicture}
\begin{axis}[
    hide axis,
    scale only axis,
    height=\figureheight,
    width=10pt,
    colormap/jet,
    colorbar horizontal,
    point meta min=1,
    point meta max=100,
    colorbar style={
        width=10cm,
        xtick={20,40,60,...,100},
        xticklabel pos=upper,
        rotate=270,
        width=5cm,
        x tick label style={xshift=0.3cm}
    }]
    \addplot [draw=none] coordinates {(0,0)};
\end{axis}
\end{tikzpicture}


==> tables/synthetic/511_table_mcmc_neff.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{2}{c}{mean($n_{eff}$)} & \multicolumn{6}{c}{$n_{eff}$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-9}
{} &             $V$ & $T$ &     $m_V$ & $\sigma_V$ & $m_{T}$ & $\sigma_{T}$ & $\sigma_{I}$ & $\sigma_{\omega}$ \\
\midrule
MCMC      &               2 &   2 &        13 &         12 &       7 &            5 &            2 &                 3 \\
MCMC(MAP) &               8 &   8 &     2,215 &      2,114 &   1,679 &        2,353 &        1,297 &             1,521 \\
\bottomrule
\end{tabular}


==> tables/synthetic/511_table_mcmc_rhat.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{2}{c}{mean($\hat{R}$)} & \multicolumn{6}{c}{$\hat{R}$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-9}
{} &             $V$ &   $T$ &     $m_V$ & $\sigma_V$ & $m_{T}$ & $\sigma_{T}$ & $\sigma_{I}$ & $\sigma_{\omega}$ \\
\midrule
MCMC      &           3.446 & 3.515 &     1.107 &      1.105 &   1.185 &        1.227 &        2.765 &             1.684 \\
MCMC(MAP) &           1.328 & 1.319 &     1.000 &      1.005 &   1.005 &        1.001 &        1.003 &             1.002 \\
\bottomrule
\end{tabular}


==> tables/testbench/511_table_mcmc_neff.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{2}{l}{mean($n_{eff}$)} & \multicolumn{6}{l}{$n_{eff}$} \\
{} &             $V$ & $T$ &     $m_V$ & $\sigma_V$ & $m_{T}$ & $\sigma_{T}$ & $\sigma_{I}$ & $\sigma_{\omega}$ \\
\midrule
MCMC      &               4 &   5 &     2,852 &        132 &   1,667 &            7 &            5 &                 6 \\
MCMC(MAP) &              45 &  49 &     2,085 &      2,138 &   1,804 &        1,985 &        1,297 &             1,237 \\
\bottomrule
\end{tabular}


==> tables/testbench/511_table_mcmc_rhat.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{2}{l}{mean($\hat{R}$)} & \multicolumn{6}{l}{$\hat{R}$} \\
{} &             $V$ &   $T$ &     $m_V$ & $\sigma_V$ & $m_{T}$ & $\sigma_{T}$ & $\sigma_{I}$ & $\sigma_{\omega}$ \\
\midrule
MCMC      &           2.257 & 1.835 &     1.003 &      1.033 &   1.000 &        1.169 &        1.270 &             1.219 \\
MCMC(MAP) &           1.036 & 1.036 &     1.000 &      1.001 &   1.003 &        1.002 &        1.001 &             1.001 \\
\bottomrule
\end{tabular}

